Generative Energy-Based Modeling of Binary Data with Hypernetworks

Binary image codes provide a common space in which to learn an energy for generation and inference. We introduce HyperIsing, a model in which a hypernetwork computes spin fields and couplings from the configuration being scored. This dependence allows for effective interactions beyond fixed pairs. We train the energy by ranking data codes against corrupted alternatives and, for labeled data, by comparing the energies assigned to candidate classes. On MNIST, the same fitted energy supports classification, class-conditional generation, joint image restoration and label inference. With the decoder and the number of latent proposals held fixed, search based on observed-pixel fidelity alone gives lower reconstruction error; joint inference returns a class estimate alongside the image. For unconditional cat-image generation, the method with the lowest feature likelihood divergence changes with the reference: pixel diffusion ranks first against original images, whereas HyperIsing ranks first against autoencoder reconstructions at settings selected on the evaluated grid. These results distinguish matching the distribution of decoded data from matching the original image distribution.

==> supp_cats_plots.tex <==
\FloatBarrier
\section{Cat-Image Sampling Maps and Distributional Diagnostics}
\label{app:cats-plots}
Figures~\ref{fig:cats16-supp}-\ref{fig:cats256-supp} add the dimensions not shown in Fig.~\ref{fig:cats-maps}. Each panel uses its own color scale. Each cell compares HyperIsing to the uniform baseline at the same dimension. The side panels average over sampled settings. The expanded views in Figs.~\ref{fig:cats-marginal-real}-\ref{fig:cats-marginal-ilmd} give the temperature and sweep-count marginals separately for all six dimensions.

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Originals}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_16_real_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Reconstructions}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_16_reco_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Validation codes}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_16_ilmd.png}\end{minipage}
\caption{16-bit cat sampling landscape. Original-reference FLD, reconstruction-reference FLD, and ILMD to validation codes. Positive improvements indicate lower values than uniform. The diffusion reference lines show the corresponding metric contrasts with uniform sampling. Each panel has its own scale.}\label{fig:cats16-supp}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Originals}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_64_real_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Reconstructions}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_64_reco_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Validation codes}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_64_ilmd.png}\end{minipage}
\caption{64-bit cat sampling landscape. Original-reference FLD, reconstruction-reference FLD, and ILMD to validation codes. Positive improvements indicate lower values than uniform. The diffusion reference lines show the corresponding metric contrasts with uniform sampling. Each panel has its own scale.}\label{fig:cats64-supp}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Originals}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_256_real_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Reconstructions}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_256_reco_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Validation codes}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/map_256_ilmd.png}\end{minipage}
\caption{256-bit cat sampling landscape. Original-reference FLD, reconstruction-reference FLD, and ILMD to validation codes. Positive improvements indicate lower values than uniform. The diffusion reference lines show the corresponding metric contrasts with uniform sampling. Each panel has its own scale.}\label{fig:cats256-supp}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{16 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_16_real_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{32 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_32_real_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{64 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_64_real_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{128 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_128_real_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{256 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_256_real_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{512 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_512_real_fld.png}\end{minipage}
\caption{Marginal trends of FLD against original images. For each dimension, the left half averages improvement over sweep counts at each temperature and the right half over temperatures at each sweep count. Bands are one standard deviation across those settings. Dashed and dotted lines identify fixed comparators. The 512-bit range includes additional temperatures.}\label{fig:cats-marginal-real}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{16 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_16_reco_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{32 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_32_reco_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{64 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_64_reco_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{128 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_128_reco_fld.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{256 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_256_reco_fld.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{512 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_512_reco_fld.png}\end{minipage}
\caption{Marginal trends of FLD against autoencoder reconstructions. For each dimension, the left half averages improvement over sweep counts at each temperature and the right half over temperatures at each sweep count. Bands are one standard deviation across those settings. Dashed and dotted lines identify fixed comparators. The 512-bit range includes additional temperatures.}\label{fig:cats-marginal-reco}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{16 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_16_ilmd.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{32 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_32_ilmd.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{64 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_64_ilmd.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{128 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_128_ilmd.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{256 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_256_ilmd.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{512 bits}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/marginal_512_ilmd.png}\end{minipage}
\caption{Marginal trends of ILMD to validation codes. For each dimension, the left half averages improvement over sweep counts at each temperature and the right half over temperatures at each sweep count. Bands are one standard deviation across those settings. Dashed and dotted lines identify fixed comparators. The 512-bit range includes additional temperatures.}\label{fig:cats-marginal-ilmd}\end{figure}


\FloatBarrier
\subsection{Reference Reconstructions and Latent Distributions}
The archival FID implementation uses Inception features \cite{heusel}; it is distinct from the MNIST CNN64 statistic and the cat DINOv2 FLD. The cat generative precision reverses the coverage question in Appendix~\ref{app:metrics}: it asks what fraction of generated features lie within neighborhoods around training-reference features \cite{recall,fldcode}. Comparing both original and reconstructed references makes explicit how a different target changes the apparent quality of a generated set (Fig.~\ref{fig:cats-extra-visual}).

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{FID to originals}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_real_FID.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{FID to reconstructions}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_reconstructed_FID.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Generative precision to originals}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_real_Precision.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Generative precision to reconstructions}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_reconstructed_Precision.png}\end{minipage}
\caption{Additional cat-image comparators. Each HyperIsing series is selected independently by the quantity shown. Inception-based FID is lower-is-better; generative precision is higher-is-better. Original and reconstruction references are reported separately.}\label{fig:cats-extra-visual}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{One-spin means}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_magnetization_rmse.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Raw pair moments}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_pair_moment_rmse.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Connected correlations}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_connected_correlation_rmse.png}\end{minipage}
\caption{Cat latent-moment components relative to validation codes. The first two quantities enter ILMD; connected correlations are reported separately. Each HyperIsing series uses the best available setting for its own metric. The train-validation contrast is a finite-sample diagnostic.}\label{fig:cats-extra-moments}\end{figure}

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{4 bits per block}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_blockwise_js_4.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{6 bits per block}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_blockwise_js_6.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{10 bits per block}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_blockwise_js_10.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{12 bits per block}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_blockwise_js_12.png}\end{minipage}
\caption{Blockwise Jensen-Shannon comparisons at alternative block sizes. The main text shows eight-bit blocks; these panels show changes in the result and its empirical scale as the block size changes. Error bars summarize variation across the sampled blocks. The selected HyperIsing settings may differ by panel.}\label{fig:cats-extra-js}\end{figure}

Figure~\ref{fig:cats-extra-diversity} reports distinct sample counts, exact training-code matches, and observed fractions of binary support. The support fraction divides the number of distinct sampled codes by $2^n$, giving a denominator that grows exponentially with code length.

\begin{figure}[!tbp]\centering
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Unique-code fraction}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_Latent_unique_fraction.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Exact training-code matches}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_Latent_match_rate.png}\end{minipage}\par\medskip
\begin{minipage}[t]{.48\linewidth}\centering \textbf{Within-set Hamming distance}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_Latent_mean_hamming.png}\end{minipage}\hfill \begin{minipage}[t]{.48\linewidth}\centering \textbf{Fraction of all possible codes}\par\smallskip \includegraphics[width=\linewidth]{figures/cats_supp/comparison_Latent_space_coverage.png}\end{minipage}
\caption{Cat latent-space diagnostics. Unique fraction counts distinct codes per sample; match rate counts generated codes equal to any training code; Hamming is the mean normalized bit difference between sampled pairs of generated codes; space fraction counts observed distinct codes divided by $2^n$. HyperIsing settings are chosen per panel.}\label{fig:cats-extra-diversity}\end{figure}


\FloatBarrier
\subsection{Fixed-Sweep Temperature Scan at 512 Bits}
Figures~\ref{fig:cats-fixed512} and~\ref{fig:cats-fixed512-visual} show latent and image-feature metrics over the 512-bit temperature scan at 128 sweeps.


\begin{figure}[!tbp]\centering
\includegraphics[width=\linewidth,height=.40\textheight,keepaspectratio]{figures/cats_supp/fixed512_energy_hamming_ilmd.pdf}
\caption{Fixed 128-sweep scan at 512 latent bits. Panels report mean energy, mean normalized pairwise Hamming distance between generated codes, and ILMD against validation codes. Distinct markers identify the extension beyond the earlier temperature range.}
\label{fig:cats-fixed512}\end{figure}

\begin{figure}[!tbp]\centering
\includegraphics[width=\linewidth,height=.84\textheight,keepaspectratio]{figures/cats_supp/fixed512_image_quality.pdf}
\caption{Image-space results for the same fixed 128-sweep scan. Columns separate original images from autoencoder reconstructions; rows show Inception FID, validation FLD, generative precision, and generative recall. Lower is better for FID and FLD, and higher is better for precision and recall.}
\label{fig:cats-fixed512-visual}\end{figure}

\FloatBarrier

